The Best Ends by the Best Means: Ethical Concerns in App Reviews

This work analyzes ethical concerns found in users' app store reviews. We performed this study because ethical concerns in mobile applications (apps) are widespread, pose severe threats to end users and society, and lack systematic analysis and methods for detection and classification. In addition, app store reviews allow practitioners to collect users' perspectives, crucial for identifying software flaws, from a geographically distributed and large-scale audience. For our analysis, we collected five million user reviews, developed a set of ethical concerns representative of user preferences, and manually labeled a sample of these reviews. We found that (1) users highly report ethical concerns about censorship, identity theft, and safety (2) user reviews with ethical concerns are longer, more popular, and lowly rated, and (3) there is high automation potential for the classification and filtering of these reviews. Our results highlight the relevance of using app store reviews for the systematic consideration of ethical concerns during software evolution.

==> abstract.tex <==
This work analyzes ethical concerns found in users' app store reviews. We performed this study because ethical concerns in mobile applications (apps) are widespread, pose severe threats to end-users and society, and lack systematic analysis and methods for detection and classification. In addition, app store reviews allow practitioners to collect users' perspectives, crucial for identifying software flaws, from a geographically distributed and large-scale audience. For our analysis, we collected five million user reviews, developed a set of ethical concerns representative of user preferences, and manually labeled a sample of these reviews. We found that (1) users highly report ethical concerns regarding inappropriate content, accountability, and discrimination, (2) user reviews with ethical concerns are longer, more popular, and lowly rated, and (3) there is high automation potential for the classification and filtering of these reviews. Our results highlight the relevance of using app store reviews for the systematic consideration of ethical concerns during software evolution.

==> background.tex <==
\section{Types of Ethical Concerns}

\label{sec:res_taxonomy}
To categorize ethical concerns found in user reviews, we use Wright's Information and Computer Technology (ICT) Ethical Impact Assessment Framework as a starting point~\cite{wright2011framework}. We chose this framework in contrast to other existing sets of ethical concerns as it focuses on ICT as a whole rather than too restricted of a domain like just AI \cite{future_2022} or too broad of a domain like all possible ethical concerns \cite{schwartz2012overview}. However, we found that some values from Wright's framework would be too academic to appear in user reviews. Because of this, we simplified some of Wright's values to reflect more vernacular ideas and language.

The values that remain unchanged from Wright's framework to our set are \textit{sustainability}, \textit{safety}, \textit{accessibility}, \textit{accountability}, and \textit{transparency}. These values were at the right level of complexity to align well with user perceptions of ethical concerns of mobile applications. For ethical concerns relating to the proper maintenance of user data, Wright had multiple more fine-grained categories. We merged these into one larger \textit{privacy} category. Wright also had multiple ethical values relating to \textit{discrimination}, which we combined into one category. We excluded four concerns mentioned in our reference literature~\cite{wright2011framework}---\textit{value sensitive design, social solidarity, inclusion and exclusion, dignity} and \textit{isolation and substitution of human contact}---from our ethical concerns set. Although these critical values warrant focus, we posited that the concepts behind them were too abstract and pedantic to be found in user reviews. Figure~\ref{fig:taxonomy_mods} shows the initial set of ethical concerns we used for our work based on Wright's framework. 

\textit{Internal and External Concerns}
\label{sec:inex}
Not only has mobile application software created ethical concerns for users in virtual spaces, but these concerns have also bled into the physical realm. Within the past few years, software companies have received flack for influencing elections, inciting real-world violence, and facilitating sexual assault~\cite{brattberg_maurer_2018}, \cite{guardian_2018}, \cite{raitanen2019deep}, \cite{lee2022storm}, \cite{o2018cnn}.
To identify and analyze these material matters, we consider any concerns which involve the physical world as \textit{external} ethical concerns. We identified six ethical concerns as potentially external: \textit{accountability, discrimination, safety, scam, sustainability, and accessibility\footnote{The scam ethical concern was added after the analysis described in Section~\ref{sec:annotation}}}. This consideration can help developers understand the scope of the ethical concern and aid them with identification and mitigation. Similarly, we consider \textit{internal} ethical concerns as those concerns that occur within the realm of the software application. For example, discriminating algorithms or end-users discriminating against each other within the software platform.  

==> design.tex <==
\section{Research Scope}
\label{sec:study_design}
The main goal of this work is to study  user reviews' ethical concerns and to understand their potential for informing software processes on ethical concerns. For this purpose, we focus on three research questions:

\textbf{(RQ1)} Which types of ethical concerns are present in user reviews on the Google Play Store?

\textbf{(RQ2)} What characteristics do user reviews with ethical concerns in the Google Play Store have?

\textbf{(RQ3)} What is the automation potential of identifying and classifying ethical concerns from the Google Play Store?

%The main research questions that guided our work are:




% Include RQ and the methodology carried out to answer each of the RQ(make subsection for each of the methodologies)

% This research has three research questions that will be answered to accomplish the research goal, namely:
% \begin{enumerate}
%     \item What ethical concerns exist in mobile software applications?
%     \item What observations can be made from user reviews that are manually annotated with ethical categories?
%     \item What is an effective automated way to detect ethical concerns in reviews?
% \end{enumerate}
% The developed taxonomy can be used as an overview of what could go wrong and could aid in the prevention of these ethical concerns. With the analysis of the manually annotated data, it can become more clear if certain patterns can be observed. \\
% \newline
% Predictive modelling is used as an automated technique to find these ethical categories in user reviews. With an automated technique, large amounts of data can be processed to find these ethical concerns faster.\\

% \subsection{Data collection}
% The reviews of the applications that were analysed in this research are Alexa, Facebook, Google Home, Instagram, Linkedin, Tiktok, Vinted, Uber, Youtube and Zoom. These applications were specifically chosen because they differ in their functionality and together they reach a large and diverse target audience.  The data used in this research is collected with Google-Play-Scraper
